ImpScore: A Learnable Metric For Quantifying The Implicitness Level of Sentence

Handling implicit language is essential for natural language processing systems to achieve precise text understanding and facilitate natural interactions with users. Despite its importance, the absence of a metric for accurately measuring the implicitness of language significantly constrains the depth of analysis possible in evaluating models' comprehension capabilities. This paper addresses this gap by developing a scalar metric that quantifies the implicitness level of language without relying on external references. Drawing on principles from traditional linguistics, we define "implicitness" as the divergence between semantic meaning and pragmatic interpretation. To operationalize this definition, we introduce ImpScore, a reference-free metric formulated through an interpretable regression model. This model is trained using pairwise contrastive learning on a specially curated dataset consisting of (implicit sentence, explicit sentence) pairs. We validate ImpScore through a user study that compares its assessments with human evaluations on out-of-distribution data, demonstrating its accuracy and strong correlation with human judgments. Additionally, we apply ImpScore to hate speech detection datasets, illustrating its utility and highlighting significant limitations in current large language models' ability to understand highly implicit content. Our metric is publicly available at https://github.com/audreycs/ImpScore.

==> sec9_limitation.tex <==
\vspace{-1mm}
\section*{Limitations}
\vspace{-1mm}
While we believe this work has great practical potential in a broad research scenarios, there are certain limitations to address.
First, despite our best efforts to collect a comprehensive dataset, the training data we collected and processed—comprising $112,580$ sentence pairs—could still benefit from expansion in size and scope.
Training on a larger and more diverse dataset could potentially yield better results.
Second, a more comprehensive user study, involving a larger number of questions and tasks, could provide a more thorough assessment of \modelname beyond the two tasks introduced in this paper.
We invite the community to further explore and analyze \modelname.


==> tables/gpt_prompt.tex <==
\begin{table}[h]
\small
\centering
    \begin{tabular}{c m{10cm}} % Removed the vertical bars for a cleaner look
    \toprule % Top horizontal line
    \textbf{Dataset} & \textbf{GPT Prompt (set as system instruction)} \\
    \midrule 
    ToxiGEN  & Generate a more explicit statement that the given hate speech implies. For example, ``it is not a good idea to be trustful of foreigners.'' $\rightarrow$ ``foreigners are not trustful.'' Don't put any prefix like ``Explicit version:'' in the output. \\
    \midrule
    DGHSD   & Generate a more explicit statement that the given hate speech implies. For example, ``it is not a good idea to be trustful of foreigners.'' $\rightarrow$ ``foreigners are not trustful.'' Don't put any prefix like ``Explicit version:'' in the output. \\
    \midrule
    Adversarial  & Generate a more explicit statement that the given hate speech implies. For example, ``it is not a good idea to be trustful of foreigners.'' $\rightarrow$ ``foreigners are not trustful.'' Don't put any prefix like ``Explicit version:'' in the output. \\
    \midrule
    Implicatures & In the given conversation, what does the response imply? Please directly generate an explicit version of the response. Don't put ``An explicit version:'' or `` $<$Explicit Response$>$:'' in the output. \\
    \midrule
    LUDWIG & In the given conversation between A and B, what does B's response imply? Please directly generate an explicit version of B\'s response. Don't put ``B:'' or ``An explicit version:'' such kinds of prefix in the output. \\
    \midrule
    ABSA &  Generate a more explicit statement the given sentence implies. Don't put any prefix like ``Explicit version:'' in the output. \\
    \midrule
    SemEval & The given statement contains irony or sarcasm. Please generate an more explicit version of the statement expressing the actual meaning. Don't put any prefix like ``Explicit version:'' in the output. \\
    \midrule
    Snarks & The given statement is sarcastic. Please generate an explicit version of the statement expressing the actual meaning. Don't put any prefix like ``Explicit version:'' in the output. \\
    \bottomrule 
    \end{tabular}
    \caption{Example of a Two-Column Table with Merged Columns using Booktabs}
    \label{table:data_prompt}
\end{table}

==> tables/user_study_result.tex <==
\begin{table}[h]
    \small
    \resizebox{\textwidth}{!}{%
    \centering
    \begin{tabular}{c|l|ccccccc}
    \toprule
     Groups & Statements  & Human 1 & Human 2 & Human 3 & Human 4 & Human 5 & \modelname & Gold Rank \\
     \toprule
    \multirow{4}{*}{$G_1$} & \textcolor{red}{[most explicit]} & 1 & & & & & \\ 
                            & \textcolor{magenta}{[explicit]} & 3 & & & & &\\ 
                            & \textcolor{cyan}{[implicit]} & 4 & & & & & \\ 
                            & \textcolor{blue}{[most implicit]} & 2 & & & & & \\ 
    \bottomrule
    \end{tabular}
    }
    \caption{Caption}
    \label{tab:my_label}
\end{table}
